Time Adaptive Gaussian Model

Multivariate time series analysis is becoming an integral part of data analysis pipelines. Understanding the individual time point connections between covariates as well as how these connections change in time is non-trivial. To this aim, we propose a novel method that leverages on Hidden Markov Models and Gaussian Graphical Models -- Time Adaptive Gaussian Model (TAGM). Our model is a generalization of state-of-the-art methods for the inference of temporal graphical models, its formulation leverages on both aspects of these models providing better results than current methods. In particular,it performs pattern recognition by clustering data points in time; and, it finds probabilistic (and possibly causal) relationships among the observed variables. Compared to current methods for temporal network inference, it reduces the basic assumptions while still showing good inference performances.

==> prediction.tex <==
Often, when analysing time series, we may want to perform prediction of future behaviour. In particular, given the time series in an interval $[n-w, n]$, we want to understand the multi-variate behaviour at $n+1$. 
%The main objective of time series models is to make predictions of their next values.
Supposing to have the complete time series $X^{N\times d}$, we consider a moving window $w$ and we denote with $(\+X,\+y)$ the input-output of the regression model, where $\+X\in \mathbb{R}^{N\times dw}$ is the original time series where we add, at each time point, $(w-1)d$ time series corresponding to the past observations in the window, and $\+y\in\mathbb{R}^{N\times d}$ %\todo{N? non d? N non e' la lunghezza di tutta la time-series} 
are the values of the original time series at $n+1$. 
Note that the regression we are performing is a multi-output regression where we aim at \textit{(a)} inferring the values of the observations at $n+1$ and \textit{(b)} understanding their relationships in terms of conditional dependency (\textit{i.e.}, the graph that connects them). \\
%Our model allows to make two types of predictions: the first one is related to the prediction of the next observation in time, while the second allows us to understand the next most probable state of the system. 
%At time $n$, to predict the next observation we consider a regression model which takes as input $(\+X,\+y)$, where $\+X\in \mathbb{R}^{N\times dp}$ are the past $p\in\mathbb{N}$ values of the time series under consideration (namely the observations in the time interval $[n-p, n]$) and the output $\+y\in\mathbb{R}^{N\times d}$ %\todo{N? non d? N non e' la lunghezza di tutta la time-series} 
%is the values at $n+1$. 
First, we apply TAGM on the augmented multi-variate time series, obtaining $K$ states and the corresponding graphs $\Theta_k \in \mathbb{R}^{dw\times dw}$ for $k=1, \dots, K$. Then, 
we consider separately each variable $j=1, \dots,d$, for which we aim at finding a function $f$ defined as %is given by % different models, one for each time series. to obtain a prediction for each time series, it is needed to train $d$ different models, one for each time series. \\
%So far \todo{name} model does not look like a regression model since it does not make distinction between input and output but it is possible to find a transformation which makes it of that form. If the input matrix of \todo{name} model is $(\+X,\+y)$, where $\+X$ and $\+y$ are respectively the matrix and the vector defined above,
%Suppose our input dataset has the form $(\+X,\+y)$, where $\+X\in \mathbb{R}^{N\times dp}$ with $p\in\mathbb{Z}^+$ represents the past features and $\+y\in\mathbb{R}^N$ is the present feature.  
%Then, for each $j=1, \dots,d$ the corresponding regression model is of the type % If we want to predict all the $d$ time series next values we will have to perform $d$ regressions of the type
\begin{equation}\label{yf}
\+y_{n+1}[j]= f(\+x_n).
\end{equation}
where $\+x_n \in \mathbb{R}^{dw}$ is the $n$-th row of the matrix $\+X$. 
%where we are using the previous $p$ observations of the $j$-th variable to perform regression.
%with $\+X[nd]\in\mathbb{R}^p$ and $y_{n+1}[d]\in\mathbb R$. 
By minimizing %\todo{? non capisco point-wise} 
the expected squared prediction error, we obtain that $f(\+x_n) = \mathbb{E}[\+y_{n+1}[j]|\+X=\+x_n]$.
%which becomes using the probability product rule
% \begin{equation}\label{Ef}
% EPE[f] = \mathbb E[Y-f(\+X)]^2 = \mathbb E_{\+X}[\mathbb E_{Y|\+X}[(Y-f(\+X))^2|\+X]]\implies f(\+x) = \mathbb{E}[Y|\+X=\+x].
%\end{equation}
Note now that the probability of $\+y_{n+1}[j]$ given  $\+x_n$ and the corresponding hidden state $\+z_n$ is a univariate Gaussian distribution \cite{mardia1979jt} defined as 
%Then, by using the Gaussian conditional distribution property \cite{mardia1979jt}, the observation $\+y_{n+1}[j]$ given  $\+x_n$ and the hidden state $\+z_n$ is obtained by
\begin{equation}\label{po}
p(\+y_{n+1}[j]|\+x_n,z_{n,k}=1) =\mathcal{N}(\bar{\mu},\bar{\sigma})
\end{equation}
where $\bar{\mu}= \mu^{k}_{\+y[j]}+(\+x-\+\mu^{k}_{\+X})\Theta^{k}_{\+X\+X}\Sigma^k_{\+X \+y[j]}$, $\bar{\sigma} = \Sigma^k_{\+y[j]\+y[j]}-(\Sigma^k_{\+X\+y[j]})^\top\Theta^{k}_{\+X\+X}\Sigma^k_{\+X\+y[j]}$ where the subscript notation indicate the matrix elements of the matrices or vectors corresponding respectively to the indices of the features $\+X$ and $\+y[j]$ 

This is an integration for the notation of the matrix block partition in Section 4 of the main document. Reminding that to transform TAGM into a regression model we consider $(\+X,\+y)$ its input-output matrix,  where $\+X\in \mathbb{R}^{N\times dw}$ and $\+y\in\mathbb{R}^{N\times d}$, where $d$  is the number of the time series and $w\in \mathbb{N}$ is the past moving window length. For each output $\+y[j]$ with $j\in\{1,\dots,d\}$, the $k$ state covariance matrix partition is
\[
\Sigma^k=\begin{pmatrix}
    \Sigma^{k}_{\+X\+X}&\+\sigma^{k}_{\+X\+y[j]}  \\
    \sigma^{k\top}_{\+X\+y[j]}& \sigma^{k}_{\+y[j]\+y[j]}  
    \end{pmatrix}
\]
where the subscript notation indicate the matrix elements corresponding respectively to the indices of the features $\+X$ and $\+y[j]$. Similar partition can be found for the precision matrix $\Theta^{k}$ and the mean vector $\+\mu^{k}$.

 %\todo{cosa vuol dire - We use the subscript notation $\+X$ and $\+y[j]$ to indicate the correlation matrix elements corresponding respectively to the features $\+X$ and $\+y[j]$}.
%\todo{credo vada esplicitato cosa intendi con la notazione a pedice delle XX e delle Xy}
Then combining Equation \eqref{po} and \eqref{yf} we get
\begin{equation}\label{predmodel}
    \+y_{n+1}[j] = \mu^{k}_{\+y[j]}+(\+x_{n}-\+\mu^{k}_{\+X})\Theta^{k}_{\+X\+X}\Sigma_{\+X\+y[j]}
\end{equation}
which corresponds to a time-varying lasso linear regression %since its parameters are $\ell_1$ regularized by the graphical lasso 
\cite{friedman2001elements}.
Note that, the regression model we just described assumes the knowledge of $k$, \textit{i.e.}, the prediction of the hidden state at $n+1$. %. cluster which the prediction belongs to and all the other parameter but $\+x_{n}$ are the results of the model fit. 
We estimate this value using the Viterbi method which is used to infer the most likely state for each observation $n$ (and, thus the corresponding precision matrix and mean) %given and as consequence of that it finds the mean vector and the covariance matrix from which each sample comes from
\cite{forney1973viterbi}.

Such method is based on the Viterbi algorithm which focuses on finding the most likely sequence of hidden states. This is not the only methods that our algorithm can perform. There are two other methods to make prediction of the next point or the next cluster.
\begin{itemize}
\item \textbf{Hassan method}: based on \cite{hassan2005stock} evaluates the value of the next point to be  equal to the next one with the most similar likelihood in the past. Therefore, it is necessary to compute all the likelihood $\mathcal{L}_{\+x_t}$ of  the entire sequence of the observations. If $t^*= \arg\min_{t\in\{1,T-1\}}\{|\mathcal{L}_{\+x_T}-\mathcal{L}_{\+x_t}|\}$ then $\+x_{T+1} = \+x_{t^*+1}$. This method can be used also to predict the next state since it would be the one corresponding to the point $ \+x_{t^*+1}$.
\item \textbf{Probabilistic method}: it inspired by the fact that we are able to compute an analytical expression of the next point probability distribution. The drawback of this method is that it is time consuming since it has to evaluate multiple-integrals whose number increases with the number of the considered time-series. From the conditional independences $\+z_{N+1}\independent\+X|\+z_N$ and $\+x_{N+1}\independent\+X|\+z_{N+1}$  the likelihood of the next point given all the observations is 
\[
p(\+x_{N+1}|\+X)= \frac{1}{p(\+X)}\sum_{\+z_{N+1}}p(\+x_{N+1}|\+z_{N+1})\sum_{\+z_{N}}p(\+z_{N+1}|\+z_{N})\alpha(\+z_N).
\]

This formula is useful because it allows to understand which are the most probable region of the input space. Moreover we can compute its expectation value and variance:
\begin{align*}
\mu_{T+1} &= \mathbb{E}[\+x_{N+1}] = \int \+x_{N+1}p(\+x_{N+1}|\+X)d\+x_{N+1}\\
 \Sigma_{T+1} &=\text{Var}(\+x_{N+1})= \int( \+x_{N+1}-\mu_{T+1})^2p(\+x_{N+1}|\+X)d\+x_{N+1}.
\end{align*}
\end{itemize}
To predict the state at $n+1$, given the output $k^*$ of the Viterbi algorithm at time $n$, we either draw the most probable state from the distribution $A[k^*]$, \textit{i.e.} the $k^*$-th transition matrix row or we assume that the state remain fixed at $k^*$.

%with the parameters of cluster $k^*$. 
%The Viterbi method can, thus, also be used as a statistical tool to analyze the covariance matrix of time-varying time series. %In fact, it allows to identify the %if someone is interested in finding the covariance matrix of the next observation, he can fit the data using our model and then apply the Viterbi algorithm to find the 
%covariance matrix corresponding to the $N$-th observation \todo{questo lo renderei piu' chiaro prima, la notazione la cambiamo un po' nel corso della sezione (the last one)}. At this point, to predict the $N+1$ covariance matrix we can either draw the most probable state from the transition matrix or keep the same state. % as the last one if he believes that the states are more \todo{static}. 
%We will show in the next sections that this technique outperforms the common way to compute the empirical covariance of the last $N$ observations.
% \textbf{Granger causality}
% The procedure above allows us to connect the graph at each state to Granger causality test \cite{granger1969investigating}. Multivariate Granger causality analysis aims at detecting those variables that across all time series are causal for other. Typically, this is achieved by fitting a VAR model \cite{granger1969investigating} on the time series. The main drawback of this model is that it assumes that all the observations are i.i.d. \ and thus that causal relations are stable in time.  TAGM, on the other hand, allows to have different causality patterns in time providing more flexibility and interpretability. Indeed, we can note that if the graph has an edge between two variables, we will then exploit that edge to perform regression on the next time point. This entails that there is a causal relationship between the two variables simply provided by the sequentiality in which they appear. Such causal relationship will change depending on the state, thus allowing to have a clearer understanding of the causal relationships among variables in time.
%Following the algorithm, we select the next most probable state by looking at the transition matrix $A$, then if $k_{n+1} = j$ we select the precision matrix related to the $j$-th state $\Theta_j$.  


%Forecasting is one of the main objectives for a machine learning model applied to time series analysis. Our model is able to simultaneously predict: (i) the next point relations between the multivariate time series in term of the precision matrix, and (ii) the values of the next point assumed by each time series.\\
% Our model can be utilized for two kinds of goals: (i) to understand how $d$ time series change in time their simultaneous reciprocal behaviour  and predict the next relationships given all the past sequences, (ii) to predict from the past $p$ values the next values with a confidence level. (i) typically is useful in finance to construct an investment portfolio which maximizes the returns minimizes the risks given the time series means and covariance. Therefore if the considered time series are time-varying the 
%empirical means and covariance may lead to unexpected portfolio outcomes. (ii) can be employed when someone wants to make prediction in a dynamical system emphasizing the most important relations between the considered time series.
%To predict (i) we exploit the  \emph{Viterbi method} 
%The state of the prediction $k_{T+1}$ can be either drawn from the transition matrix or  $k_{T+1}= k_{T}$ . Therefore the precision matrix $\Theta_{T+1}= \Theta_{k=k_{T+1}}$.  
%There are other possible prediction methods, they are described in Section 5 - Supplementary material.\\
%\begin{enumerate}
%\item 
%\item \textbf{Hassan method}: it is based on \cite{hassan2005stock}. The state of the next point is equal to the next one with the most similar likelihood to today in the past.Therefore, it is necessary to compute all the likelihood $\mathcal{L}_{\+x_t}$ of the the entire sequence of the observations. If $t^*= \arg\min_{t\in\{1,T-1\}}\{|\mathcal{L}_{\+x_T}-\mathcal{L}_{\+x_t}|\}$ then $\+x_{T+1} = \+x_{t^*+1}$.
%\item \textbf{Probabilistic method}: from the conditional independences $\+z_{N+1}\independent\+X|\+z_N$ and $\+x_{N+1}\independent\+X|\+z_{N+1}$ it is possible to prove that
%\begin{equation}
%p(\+x_{N+1}|\+X)= \frac{1}{p(\+X)}\sum_{\+z_{N+1}}p(\+x_{N+1}|\+z_{N+1})\sum_{\+z_{N}}p(\+z_{N+1}|\+z_{N})\alpha(\+z_N)
%\end{equation}
%which is the pdf of the next point$\+x_{N+1}$ given all the observed data $\+X$. Then
%\begin{align}
%\mu_{T+1} &= \mathbb{E}[\+x_{N+1}] = \int \+x_{N+1}p(\+x_{N+1}|\+X)d\+x_{N+1\label{mupred}}\\
% \Sigma_{T+1} &=\text{Var}(\+x_{N+1})= \int( \+x_{N+1}-\mu)^2p(\+x_{N+1}|\+X)d\+x_{N+1}.\label{sigmapred}
%\end{align}
%From  \eqref{mupred} and \eqref{sigmapred} we get a mean value and a confidence interval as in the Viterbi method.
%\end{enumerate}
%\begin{figure}[ht]
%\begin{center}
%\caption{HMM-GGM prediction example}
%\label{Fig_PredHMMGGM}
%\includegraphics[width=0.4\textwidth]{HMM_GMM_pred2}
%\end{center}
%\end{figure}
%For prediction (ii) we basically perform regression using past observations as feaures and predicting the future observation. 
%%connecting the past observations to one of the present observation. Therefore 
%The input dataset has the form $(\+X,\+y)$ where $\+X\in \mathbb{R}^{N\times dp}$ and $\+y\in\mathbb{R}^N$ with $p\in\mathbb{Z}^+$ is the window number of past observations that we decide to consider for the regression task. For each $j=1, \dots,d$ we need to perform a regression of the type % If we want to predict all the $d$ time series next values we will have to perform $d$ regressions of the type
%\begin{equation}\label{yf}
%y_{n+1}[j]= f(\+X[nj])
%\end{equation}
%where we are using the previous $p$ observation of the $j$-th variable to perform regression.
%%with $\+X[nd]\in\mathbb{R}^p$ and $y_{n+1}[d]\in\mathbb R$. 
%One of the possible methods to find it is to minimize pointwise the expected squared prediction error, which gives us that $f(\+x) = \mathbb{E}[Y|\+X=\+x]$
%%which becomes using the probability product rule
%% \begin{equation}\label{Ef}
%% EPE[f] = \mathbb E[Y-f(\+X)]^2 = \mathbb E_{\+X}[\mathbb E_{Y|\+X}[(Y-f(\+X))^2|\+X]]\implies f(\+x) = \mathbb{E}[Y|\+X=\+x].
%%\end{equation}
%Then, by using the Gaussian conditional distribution property in \cite{mardia1979jt}, the observation $y_{n+1}$ given $\+x_n$ and the hidden state $\+z_n$ is obtained by
%\begin{equation}\label{po}
%p(y_{n+1}|\+x_n=\+x,z_{n,k}=1) =\mathcal{N}(\mu^{\text{pred}},\sigma^{\text{pred}})
%\end{equation}
%where $\mu^{\text{pred}}= \mu^{k}_{Y}+(\+x-\+\mu^{k}_{\+X})\+\Theta^{k}_{\+X\+X}\+\sigma^k_{\+X Y}$, $\sigma^{\text{pred}}= \+\sigma^k_{\+XY}-\+\sigma^k_{\+XY}\+\Theta^{k}_{\+X\+X}\+\sigma^k_{\+XY}$ and we have partitioned the correlation matrix $\+\Sigma^{k}= 
%\begin{pmatrix}
%\+\Sigma^{k}_{\+X\+X}&\+\sigma^{k}_{\+XY}  \\
%\+\sigma^{k\top}_{\+XY}& \+\sigma^{k}_{YY}  
%\end{pmatrix}$, similarly for $\+\Theta^{k}$ and $\+\mu^{k}$. Then by \eqref{po},\eqref{Ef} and \eqref{yf} we get
%\begin{equation}
%y_{n+1} = \mu^{k}_{Y}+(\+x_{n}-\+\mu^{k}_{\+X})\+\Theta^{k}_{\+X\+X}\+\sigma_{\+XY}
%\end{equation}
%where $k$ can be found using the Viterbi method described above and all the other parameter but $\+x_{n}$ are the results of the model fit.
%
%
%Note that the above equation is linear in $\+x_n$ and therefore our model produce a Gaussian linear dynamical regression. Moreover with this problem formulation it is also possible to infer causal relations between the past variables  $\+X^{\text{past}}$ and $X^{\text{out}}$. In fact from the probabilistic interpretation of the precision matrix $\+\Theta^{k}_{i,j} =p(X_j|X_i)$ we can say that $X^{\text{past}}_i$ causes $X^{\text{out}}$ with probability $\+\Theta^{k}_{X^{\text{past}}_i,X^{\text{out}}}$. Therefore, if $\+\Theta^{k}_{X^{\text{past}}_i,X^{\text{out}}}=0$ then there is no causal relation between $X^{\text{past}}_i$ and $X^{\text{out}}$.
%
% \subsubsection{Aternative way to compute $\Theta_{k}$}
%
% We would like to fix the hyperparameter $\lambda$ using the same choice in \cite{banerjee2008model}. In this case we have to pay attention to the fact that the empirical variance and the number of samples depend on the cluster $k$. To emphasize that the penalty parameter depends on the cluster $k$ we will add a subscript to $\lambda$. Adapting the formula in  \cite{banerjee2008model} we have
% \begin{equation}\label{lambkal}
% \lambda_k( \alpha)= \max_{i>j}\{\hat{\sigma}^k_i\hat{\sigma}^k_j\}\frac{t_{n_k-2}(\frac{\alpha}{2d^2})}{\sqrt{n_k-2+t^2_{n_k-2}(\frac{\alpha}{2d^2})}}
% \end{equation}
% where $\alpha\in [0,1]$ is the confidence level, $ \hat{\sigma}^k_i$ is the empirical variance of the node ( feature ) $i$ for state $k$ which is given by
% \[
% \hat{\sigma}^k_i= \sum_{n=1}^N \gamma(z_{n,k})(X_{i,i}^n-\mu^k_{i})^2,
% \]
% the function $t_{n_k-2}(\cdot)$ is the Student's t-distribution for $n_k-2$ degrees of freedom and finally $n_k =\lfloor \sum_{n=1}^N \gamma(z_{n,k}) \rfloor$. If $n_k<3$ then $\lambda_k( \alpha)=0$.  
%
% Substituting \eqref{lambkal} into \eqref{Qthk}, after some calculations we obtain the same expression with a different  $\Tilde{\lambda}_k$ which is given by
% \[
% \Tilde{\lambda}_k= \max_{i>j}\{\tilde{S}^k_{i,i}\tilde{S}^k_{j,j}\}\frac{t_{n_k-2}(\frac{\alpha}{2d^2})}{\sqrt{n_k-2+t^2_{n_k-2}(\frac{\alpha}{2d^2})}}
% \]

==> real_data.tex <==
TAGM can be employed to construct an investment portfolio and to predict future prices of financial data. We consider three securities (\textit{i.e.} tradable financial assets): Petrobras (PETR4), WTI crude Oil front futures and exchange from US dollar to Brazilian Real (USD/BRL).
These three securities have deep investment connections and being able to construct a balanced portfolio assigning the right weight to each of them would allow us to obtain profits. 
%
%correctly invest in one of the three would allow us to obtain profit. 
%
%In this section we apply our model and the methods that we have already tested with synthetic data to a real dataset. We choose to construct a portfolio with three securities: Petrobras (PETR4), WTI crude Oil front feature and the exchange from US dollar to Brazilian Real (USD/BRL). The idea behind this portfolio is that  Petrobras is a brazilian energy company specialized in the petroleum sector, therefore it is correlated with the WTI oil price movement and since the WTI is priced in US dollar and Petrobras in Brazilian Real the exchange between the two currencies is important when someone wants to buy or sell one and the other. 
%

\textbf{Building an investment portfolio}
We consider the period from 12/01/2010 to 15/09/2016, corresponding to 1635 trading days which have many price swings (up and down) (see Figure \ref{fig:investment_real_data} left panel) that are suitable to show how TAGM can be successfully employed to invest. We train our model on the first 1470 days and we test on the last 165 (from 20/01/2016 to 15/09/2016). In the evaluation we suppose for simplicity that there are no trading fees. 
The goal for portfolio construction is finding
%he is not interested  in the next $n$ day value predictions but 
%we aim at finding 
a combination of weights for each security which allows us to earn a positive return in the long run and being backed from big losses in case of price oscillations. According to the Markowitz mean-variance portfolio optimization theory \cite{Board2001} the two quantities which are needed to construct a portfolio with the above characteristics are: the expected value of returns and their covariance. The issue with these two quantities for prices is that they may vary in time and therefore every time they vary the portfolio weights should vary accordingly. This is the reason why TAGM is suitable to perform portfolio optimization even if the time series relations are time-varying. We compare the performance of the portfolio in terms of profits and losses (P\&L) by adopting the strategy based on 
%with the one constructed through the empirical covariance and the expected returns of the 
last 50 days covariances and  expected returns  and the ones estimated by TAGM. The results in terms of  P\&L percentage variation are shown in Figure \ref{fig:investment_real_data} central panel where it is possible to see how TAGM outperforms the empirical covariance. This is due to the changes in trend of the WTI Crude Oil security, which can be captured by TAGM but not by the mean empirical covariance strategy.
% In particular, if we look at the time-series evolution during the trading days we see that the blue and the red lines have respectively downward and upward trend while the green line changes trend during this period. This means that the covariance has to be changed as well. Therefore the \todo{name} model, as expected, was able to adapt to these new situations and take advantage from them while the empirical covariance was not able to do the same.
%
%
%
%and we wanted to test how our model is able to adapt to this kind of situation . W
%\todo{Non chiaro, spiegare meglio questo paragrafo To build the portfolio we predict the next post probable state and then 
%We use the Viterbi method to compute the means and covariance of the next day and the corresponding portfolio weights from the Markowitz mean-variance portfolio optimization theory \cite{Board2001} with fixed return and minimizing over the risk (variances). We adapt our portfolio weights every time the model changes state. We compare our results with the Markowitz optimal port folio computed using the empirical means and the covariance of the previous 50 trading days. We recompute the empirical means and the covariance every 10 trading days and eventually adapt the portfolio weights. }
%The results in term of profit and loss capital percentage variation are shown in Figure \ref{fig:investment_real_data} central panel. \todo{commento sui risultati}

\textbf{Prediction of future prices}
To test TAGM regression performance on real data we considered a period of 30 trading days from 4/08/2016 to 15/09/2016. We compare our results with the same state-of-the-art regression methods used in synthetic experiments. Figure \ref{fig:investment_real_data} right panel shows that the performance of all the considered methods are very closed to each other, with TAGM slightly outperforming. This is due to the fact that past price values are not very informative to predict the next values since their short-run movements depend on the real time news and market sentiment. Therefore, as long as we do not introduce this information in the prediction it would be difficult to evaluate the prediction performance as all methods catch the same information (typically just noise).



\begin{figure}[t]
\centering

\includegraphics[width=\textwidth]{real_data}
% \resizebox{0.24\textwidth}{!}{
% %\begin{adjustbox}{center, width=0.24\textwidth}  
%     \begin{tabular}{l|c}
%         \toprule
%         {} &   MAE    \\
%         \midrule
%         HMM-GGM &    \textbf{0.459}$\pm$ \textbf{0.371}\\
%         Kernel RBF &  $0.462 \pm 0.380$\\
%         LSTM &   $ 0.461 \pm 0.412$    \\
%         VAR & $0.460 \pm 0.386$ \\
%         Lgb&    $0.459 \pm 0.396$         \\
%         \bottomrule
%         \end{tabular}
%         }
       
%\end{adjustbox}

\caption{Financial portfolio P\&L behaviour. On the left panel the data we analyzed, in the middle the results obtained using TAGM or the state-of-the-art method for the construction of the investment portfolio, on the right the forecasting results for the-next-time-point values of the securities.
}
\label{fig:investment_real_data}
\end{figure}


% \begin{table}
% \begin{tabular}{l|ccccc}
% \toprule
% {} &         HMM-GGM &      Kernel RBF &             LSTM &             VAR &              Lgb \\
% \midrule
% MAE &  \textbf{0.459}  $\pm$ \textbf{0.371} &  $0.462 \pm 0.38$ & $ 0.461 \pm 0.412$ &  $0.460 \pm 0.386$ &  $0.459 \pm 0.396$ \\
% \bottomrule
% \end{tabular}
% \caption{\todo{to fill}}
% \label{tab:results_prediction_real}
% \end{table}

==> synthetic_experiment.tex <==
In order to evaluate the performance of TAGM and its extensions we devised three sets of experiments. 

\paragraph{Data generation}
For all of them we generated synthetic data, fixing the number $K$ of states. For each state $k=1, \dots, K$, the mean $\mu_k$ is drawn from normal distribution $\mathcal{N}(\+0, \mathcal{I})$, while the precision matrices $\Theta_k$ is generated by an algorithm which generates sparse semi-positive matrices  

a sequence of hidden states by sampling from a transition matrix $A$ where each row is sampled from a Dirichlet distribution. 
Given the sequence of states and the related distribution parameters we draw a sequence of $N$ samples in $d$ dimensions. We typically draw $N=2000$ observations as it resembles the number that we have in real-world domains.

\todo{Real world time-series behaviour have a deep dependence on the sequence in which they appear and the relations among them can change in time. For these reasons we generate synthetic data which are tied together by a Markov process which controls the probability to remain in the same state or to go from one state to another one. To not have a sudden transition from one state to another, we define the variable $S_t$, the \textit{smooth transition} variable, which counts the number of steps necessary to go from state $i$ to state $j$, with $i\not = j$ and $i,j\in \{1,\dots,K\}$.
%
The synthetic data generation comprehend the following steps:
\begin{enumerate}
    \item we fix suitable values for:
    \begin{enumerate}
        \item \textbf{N}: the number of observations;
        \item \textbf{K}: the number of states;
        \item \textbf{d}: the number of multivariate time series;
    \end{enumerate}
    \item for every state $k\in K$, in our implementation we allow for several combinations of distributions to generate the observations. The idea is to study the behavior of the algorithm in many peculiar cases when the labels are known and from this experience try to interpret the behavior in the real dataset case when the labels are unknown.
    \begin{enumerate}
        \item The mean can be drawn in two ways 
	\begin{enumerate}
		\item if someone wants to generate means which are close to zero like in the stock return case he can pick the \textit{normal 						distribution} case with $\+\mu_k\sim \mathcal{N}(\+0, \mathcal{I}$), where $\mathcal{I}$ is the identity matrix;
		\item otherwise, \textit{uniform distribution} case with $\+\mu_k\sim \mathcal{U}(a,b)$ and $a,b \in \mathbb{R}$ with $a<b$. If $a\ll b$
			then the generated cluster are more likely to be separated between each other.  
	\end{enumerate}
        \item  The covariance matrix $\Sigma_k$ can be set  in three ways: 	
	\begin{enumerate}
        \item generating the precision matrix similarly to what was proposed in \cite{meinshausen2006high,yuan2012discussion}, fixing a certain maximum degree for each node $d$, we randomly selected its neighbours and put deterministically the weights of the edges to $0.98/d$ to ensure positive definiteness of the resulting precision matrix;
    	\item from the tool \textbf{scikit-learn.datasets} which generates a random symmetric, positive-definite matrix; 
		\item from the precision matrix stressing the links between nodes, starting from the identity matrix and putting randomly ones in the off-diagonal places respecting the symmetric matrix constraint. In this way we are generating precision matrix with either strong links between nodes or no links at all. This case is interesting because in this way the networks corresponding to each state $k$ are very different between each others like the case with means very far away.
	\end{enumerate}
    \end{enumerate}
   \item  each row of the transition matrix $A$ is generate from a Dirichlet distribution Dir$(\+\alpha)$ where $\+\alpha\in \mathbb{R}_+^{K}$. In particular, to not have too quick transitions from one state to another we impose $\alpha_i= \kappa\cdot \alpha_j$ with $i\not=j$ where $i$ is the index of the row transition we are drawing and $\alpha_j$ all the other element of $\+\alpha$ different than $\alpha_i$. $\kappa$ is also known  as the \textit{force} constant, in the sense that the bigger $\kappa$ is the more likely the state $i$ is respect to the others;
   \item at each step $n$ the state $k$ is drawn from the transition matrix $A$ then the data are drawn from the normal distribution $\+X_n\sim\mathcal{N}(\+\mu_k,\Sigma_k)$.
\end{enumerate}
From the above description it is possible to note that the introduction of the variable $S_t$ gives the freedom to create different kind of datasets according to their transition between states. Moreover, if we fix $S_t = \Bar{S}_t$  during the transition from state $i$ to state $j$ the data will be drawn from a weighted sum of the parameters which characterise the two states. If during this transition a third state is drawn then the weights will be recalibrated for the three states and so on.
%
So our datasets will differentiate according to $S_t$ and how we define the transition weights. In particular, we have:
%
\begin{enumerate}
    \item the \textbf{sudden transition} dataset: where $S_t=1$ fixed and therefore we have no smooth transition;
    \item the \textbf{fixed smooth transition} dataset: where $S_t=\Bar{S}_t\in\mathbb{Z}_+$ always and the weighted sum will take into account how many consecutive steps travelling to the destination we have done so far;
    \item the \textbf{random smooth transition} dataset: where $S_t=\Bar{S}_t\sim \mathcal{U}(a,b)$, with $a,b>1$ and $b>a$. The weights will be set as in 2. but if during a transition another state is drawn then the $\Bar{S}_t$ in this case will replace the previous one and the weights will be recomputed from the latter;
     \item the \textbf{random smooth transition and random weights} dataset: the setting is as in 3. But the weights in this case are drawn randomly from Dir$(\+\alpha)$ with $\+\alpha$ is a vector of $1$s.
\end{enumerate}}



%
%The model that we have just described and the experiments that we will show below are implemented in a fast scikit-learn compliant Python within a large library for the inference of graphical models\footnote{\texttt{link-omitted-for-anonimity}}. 
%We validate our model through synthetic data which are generated, given $K$ states, by 


\paragraph{Model selection}
Our model has two hyper-parameters to cross-validate:
\begin{enumerate}
\item the number of finite states $K$;
\item the regularization parameter $\lambda$ which regulates the sparsity of the precision matrix $\Theta_k$;
\end{enumerate}
For all experiments we cross-validated the parameters using BIC scores \cite{schwarz1978} and we performed multiple initializations to overcome the non-convexity of the problem.

To determine the number of hidden states we use the BIC approach  \cite{schwarz1978} which has the form
\[
\text{BIC}(m)= \ln\+p(\+X|m,\theta)-\frac{\nu}{2}\ln(n).
\]
$\nu$ represents the number of free parameters and  $m$ the considered model. In our case the number of free parameters can be computed in the following:
\begin{itemize}
\item the probabilities $\pi$ have dimension $K$ with one constraint, so $\nu_{\pi}=K-1$;
\item the transition matrix $A$ has dimension  $K\times K$ but each row has a constraint, so $\nu_{A}=K(K-1)$;
\item the means $\mu$ are $K$ with dimension  $d$ without any constraint, so $\nu_{\mu}=Kd$;
\item the precision matrices $\Theta$  are $K$, one for each state, with dimension $d\times d$ but they have the constraint given by graphical lasso therefore $\nu_{\Theta} = \sum_{i\geq j} e_{i,j}$ where $e_{i,j}= 0$ if $\hat{\Theta}_{i,j}=0$  and $e_{i,j}= 1$ otherwise. $\hat{\Theta}$ is the estimated precision matrix.
\end{itemize}
Putting all together the total number of free parameter $\nu$ is 
\[
\nu = \nu_{\pi}+\nu_{A}+\nu_{\mu}+\nu_{\Theta} =(K-1)(K+1)+Kd+\sum_{k=1}^K\nu_{\Theta_k} .
\]
\end{itemize}


\item {Initialization choices}
The EM algorithm requires an initialization of the parameters $\theta_{old}$. Since the likelihood function we are considering is non-convex the parameters initialization is crucial to find the optimal solution.  In particular,given the cluster number $K$ we have to initialize four parameters: the transition matrix $A$ and the initial probabilities $\+\pi$ and the Gaussian distribution parameters $\+\Theta$ and $\+\mu$.
In our implementation \footnote{\texttt{https://github.com/veronicatozzo/regain/tree/HMM}} we adopt the  following initializations choices:
\begin{itemize}
    \item \textbf{the transition matrix $A$ and the initial probabilities $\+\pi$} can either be initialised with equal probabilities for each state $\frac{1}{K}$ or by randomly sampling from a uniform distribution  $\mathcal U(0,1)$ or Dirichlet distribution Dir$(1s)$, with the constraints that each row has to sum to one;
    \item \textbf{the Gaussian distribution parameters $\+\Theta$ and $\+\mu$} are initialized by computing an  initial subdivision of the time points into clusters. In literature, the most common way is through the K-means, or  Gaussian mixture model (GMM) --- given its similarity with HHM. Both GMM and K-means are non-convex, thus, depending on initialisation lead to different solutions as well. 
    Given the dataset initial subdivision, we compute respectively the empirical covariances and means. Finally we run the graphical lasso to compute the corresponding precision matrix and we use that as initial parameters.
\end{itemize}


\paragraph{Evaluation metrics}
We compare the results in terms of V-measure for clustering performance \cite{rosenberg2007v}, Matthews correlation coefficient (MCC) for network inference performance \cite{matthews1975comparison} where we map the inferred graph precision matrix into a binary class matrix (0 no edge identified, 1 edge identified) and Mean Absolute Error (MAE) for prediction. Further details about the evaluation metrics are in Sections 5 - Supplementary.
We use a metric score for each of the following aspects:
\begin{enumerate}
\item \textbf{clustering performance}: we compare the clustering results in terms of V-measure \cite{rosenberg2007v} which return a value $v\in[0,1]$ where $v=0$ means that the cluster labels are assigned completely randomly while $v=1$ means that there is a perfect match between the true labels and the one found by the models. 
\item \textbf{network inference performance}: in order to evaluate the performances of the methods we need to identify a map between the true clusters and the identified ones in order to compare the underlying graphs. Such map is obtained by taking the maximum per row of the contingency table of the true and predicted labels. 
We then consider the true and inferred graphs as binary classes (0 no edge identified, 1 edge identified) and we compute the Matthews correlation coefficient (MCC) \cite{matthews1975comparison} which return a value in the interval$[-1,1]$ where $0$ corresponds to chance.
\end{enumerate}


